Early-Bird Diffusion: Investigating and Leveraging Timestep-Aware Early-Bird Tickets in Diffusion Models for Efficient Training

Training diffusion models (DMs) requires substantial computational resources due to multiple forward and backward passes across numerous timesteps, motivating research into efficient training techniques. In this paper, we propose EB-Diff-Train, a new efficient DM training approach that is orthogonal to other methods of accelerating DM training, by investigating and leveraging Early-Bird (EB) tickets -- sparse subnetworks that manifest early in the training process and maintain high generation quality. We first investigate the existence of traditional EB tickets in DMs, enabling competitive generation quality without fully training a dense model. Then, we delve into the concept of diffusion-dedicated EB tickets, drawing on insights from varying importance of different timestep regions. These tickets adapt their sparsity levels according to the importance of corresponding timestep regions, allowing for aggressive sparsity during non-critical regions while conserving computational resources for crucial timestep regions. Building on this, we develop an efficient DM training technique that derives timestep-aware EB tickets, trains them in parallel, and combines them during inference for image generation. Extensive experiments validate the existence of both traditional and timestep-aware EB tickets, as well as the effectiveness of our proposed EB-Diff-Train method. This approach can significantly reduce training time both spatially and temporally -- achieving 2.9$\times$ to 5.8$\times$ speedups over training unpruned dense models, and up to 10.3$\times$ faster training compared to standard train-prune-finetune pipelines -- without compromising generative quality. Our code is available at https://github.com/GATECH-EIC/Early-Bird-Diffusion.

==> Sections/7-SupplementaryMaterials.tex <==
\clearpage
\appendix

\input{tables/sm_ablation_pseudo_epoch}

\section{More Results for Finding EB Tickets}
\label{sec:existence_eb_tickets}

To provide further empirical evidence for identifying EB tickets in diffusion models, in Figure~\ref{fig:eb_taeb_heatmaps} (a) we present visualizations of pairwise mask distances across four dataset-model pairs: CelebA~\cite{celeba} LSUN Church~\cite{lsun} and LSUN Bedroom~\cite{lsun}, utilizing Denoising Diffusion Probabilistic Models (DDPMs)~\cite{ho2020denoising}, as well as ImageNet-1K~\cite{deng2009imagenet}, using the Latent Diffusion Model (LDM)~\cite{rombach2021highresolution}. For all settings, we apply magnitude-based structural pruning with a pruning rate of 50\%.

Due to the large number of training samples, we adopt a ``pseudo-epoch'' of 1K steps/iterations to expedite the identification of EB tickets in the case of LSUN Church, LSUN Bedroom, and ImageNet-1K.
The $(i,j)$-th element represents the Hamming distances between the pruned subnetworks extracted at the $i$-th and $j$-th pseudo-epochs. 

Lighter colors correspond to lower inter-mask Hamming distances, darker colors indicate higher distances. The epoch/pseudo-epoch where the EB ticket is identified is marked in red font. Unless otherwise stated, we use a convergence threshold of $\epsilon=0.1$ and a FIFO queue of length 5 for these visualizations. The results demonstrate that EB tickets are consistently identified during the early stages of training.
This set of visualizations further empirically confirms the existence of EB tickets in diffusion model training.

% speed table
\input{tables/sm_speed_table}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.68\textwidth]{Figures/eb_taeb_heatmaps_v12.pdf} % Adjust width as needed
    \caption{(a) Visualizations of pairwise Hamming distance matrices of EB tickets for the CelebA~\cite{celeba}, LSUN Church~\cite{lsun}, LSUN Bedroom~\cite{lsun}, and ImageNet-1K~\cite{deng2009imagenet} datasets when using structural magnitude pruning at pruning rate of 50\%. (b) Visualizations of Hamming distance matrices of TA-EB tickets when using structural magnitude pruning with pruning rates of 30\%, 60\%, and 80\% across timestep periods of 0-260, 240-460, and 440-1000, respectively.} 
    \label{fig:eb_taeb_heatmaps} % Optional label for referencing
\end{figure*}

\section{More Results for Finding TA-EB Tickets}
\label{sec:existence_ta_eb_tickets}

To provide further empirical evidence for identifying TA-EB tickets, we present visualizations of pairwise mask distances across four dataset-model pairs in Figure~\ref{fig:eb_taeb_heatmaps} (b): CelebA~\cite{celeba}, LSUN Church~\cite{lsun}, and LSUN Bedroom~\cite{lsun}, all utilizing the DDPM~\cite{ho2020denoising}, as well as ImageNet-1K~\cite{deng2009imagenet}, using the LDM~\cite{rombach2021highresolution}.
For these experiments, we use magnitude-based structural pruning with pruning rates of 30\%, 60\%, and 80\%, respectively. 
Similar to the case of EB tickets (Section~\ref{sec:existence_eb_tickets}), we adopt a ``pseudo-epoch'' approach for LSUN Church, LSUN Bedroom, and ImageNet-1K datasets to identify TA-EB tickets more efficiently. 

The $(i,j)$-th element of each matrix represents the Hamming distance between subnetworks pruned at the $i$-th and $j$-th pseudo-epochs across the designated timestep regions. Lighter colors correspond to lower inter-mask Hamming distances, darker colors indicate higher distances. The epoch/pseudo-epoch where the TA-EB ticket is identified is marked in red font. Unless otherwise stated, we use a convergence threshold of $\epsilon=0.1$ and a FIFO queue of length 5 for these visualizations. 
The results show that TA-EB tickets are consistently identified during the early stages of training, further confirming their existence in diffusion model training.



\section{Ablation Study on Pseudo-Epoch Choices}
\label{sec:ablation_pseudo_epoch}

We conduct ablation studies to evaluate the impact of the number of iterations per pseudo-epoch on drawn tickets' performance. We employ magnitude-based structural pruning to prune DDPMs~\cite{ho2020denoising}, using the LSUN Church dataset~\cite{lsun} as a representative case. All training hyperparameters are consistent with those in~\cite{diffPruning}, and we use 100 DDIM~\cite{song2020denoising} timesteps to generate images. 
Table~\ref{tab:sm_ablation_pseudo_epoch} presents results examining the effect of varying the number of iterations within a single pseudo-epoch, ranging from 100 to 5K. To provide a robust comparison, we also include results for a pruned network trained from scratch, which involves pruning a fully trained network to establish its connectivity and subsequently reinitializing it with random weights for training. As prior work~\cite{diffPruning} indicates, training pruned networks from scratch is highly competitive, making this a critical baseline for analysis.
We observe that the EB tickets identified in our experiments are not sensitive to the choice of pseudo-epoch, as the pseudo-epoch choice marginally impacts the final image generation quality. In all cases, we achieve a 13.88$\sim$19.78 lower FID as well as 3.09$\times$ speedups compared to the ``scratch'' baseline.

\section{Comparison with State-of-the-Art Efficient Training Methods}
\label{sec:comparison_sota}

Our EB-Diff-Train (EB) and EB-Diff-Train (TA-EB) strategies are efficient training methods designed for pruned models. Importantly, our approach is orthogonal to existing state-of-the-art (SOTA) timestep resampling techniques and can be combined with those methods to achieve more benefits. 
To validate this, we compare and demonstrate how EB-Diff-Train (EB) and EB-Diff-Train (TA-EB) can be integrated with a SOTA timestep resampling method, SpeeD~\cite{wang2024closer}. In Table~\ref{tab:speed_comparison}, we compare these methods against both unpruned models and the ``scratch'' baseline introduced in Section~\ref{sec:ablation_pseudo_epoch}. The results show that our EB-Diff-Train (EB) and EB-Diff-Train (TA-EB) methods can be applied on top of SpeeD effectively, leading to reduced FID scores of 2.40$\sim$3.28, as well as speedups of 3.45$\times$ and 6.10$\times$, respectively, compared to the ``scratch'' baseline.

\begin{figure}[b]
    \centering
    \vspace{-1.5em}
    \includegraphics[width=\columnwidth]{Figures/extra_generations_rebuttal_v2.pdf}
    \vspace{-2em}  
    \caption{More samples from the CelebA dataset. a) Generations from an unpruned model. b) Generations from a ``scratch" model with 50\% pruning rate. ``Scratch" is as defined in Section 5.1. c) Generations from our EB-Diff-Train (EB) method with 50\% pruning rate. d) Generations from our EB-Diff-Train (TA-EB) method with a 64\% average pruning rate.}
    \vspace{-1em}
    \label{fig:extra_generations_celeba}
\end{figure}

\section{Additional Generations}
\label{sec:additional_generations}
To further qualitatively show the efficacy of our EB-Diff-Train (EB) and EB-Diff-Train (TA-EB) strategies, we present additional generations using the DDPM~\cite{song2020denoising} model on the CelebA~\cite{celeba} dataset in Fig.~\ref{fig:extra_generations_celeba}. For these experiments, we compare an unpruned model, a model trained under the ``scratch'' conditions at a 50\% pruning rate, our EB-Diff-Train (EB) method with a 50\% pruning rate, and our EB-Diff-Train (TA-EB) method with a 64\% average pruning rate. The results further support that our method not only can maintain similar FID scores to the unpruned models while enjoying up to 6.74$\times$ speedup, but also maintain image fidelity qualitatively.


\begin{table}[t]
    \centering
    \caption{Additional experiments on ImageNet-1K~\cite{deng2009imagenet} using the DiT~\cite{Peebles2022DiT} model. The best FID and training speed-up are \textbf{bolded}. The number of iterations for the \textbf{TA-EB} methods are recorded as the total number of iterations for the subnetwork of longest training time.}
    \label{tab:dit_imagenet}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{lccccc}
            \toprule
            \multicolumn{6}{c}{\textbf{DiT @ ImageNet-1K 256$\times$256}} \\
            \textbf{Method} & \textbf{\#Params $\downarrow$} & \textbf{MACs $\downarrow$} & \textbf{FID $\downarrow$} & \textbf{Iters} & \textbf{Speed-Up} $\uparrow$\\
            \midrule
            Unpruned & 675.1M & 118.7G & 28.12 & 100K & 1.00$\times$\\
            \midrule
            Scratch  & 337.5M & 57.0G  & 58.23 & 100K & 0.72$\times$ \\
            \textbf{EB}    & 337.5M & 57.0G  & \textbf{33.16} & 100K & 2.63$\times$\\
            \textbf{TA-EB} & 242.1M & 40.7G  & 52.10 & 40K  & \textbf{3.11}$\times$\\
            \bottomrule
        \end{tabular}
    }

\end{table}

\section{Additional Experiments on DiTs}
\label{sec:additional_generations}
As the Diffusion Transformer (DiT~\cite{Peebles2022DiT}) is a common type of diffusion model, we include experimental results of our methods in Table~\ref{tab:dit_imagenet} using the ImageNet-1K~\cite{deng2009imagenet} dataset. For these experiments, we compare the unpruned model, a model trained under the ``scratch'' conditions at a 50\% pruning rate, our EB-Diff-Train (EB) method with a 50\% pruning rate, and our EB-Diff-Train (TA-EB) method with a 64\% average pruning rate. We see that our method can reduce the FID by $6.13\sim 25.07$ while yielding a speed-up of $3.64\times\sim 4.32\times$ as compared to the ``scratch" baseline.




==> tables/ablation_num_models.tex <==
\begin{table}[h!]
    \centering
    \vspace{-1em}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
    \multicolumn{7}{c}{\textbf{DDPM @ CIFAR10 32$\times$32}} \\
    \textbf{\#Regions} & \textbf{Avg. Pruning Rate} & \textbf{\#Params $\downarrow$} & \textbf{MACs $\downarrow$} & \textbf{FID $\downarrow$} & \textbf{Iters} & \textbf{Speed-Up $\uparrow$} \\
    \midrule
    1 Region  & 0\%   & 35.7M & 6.1G & 5.15 & 800K & 1.00$\times$ \\
    \midrule
    2 Regions & 64.2\% & 7.4M  & 1.4G & 7.37 & 200K & 6.30$\times$ \\
    3 Regions & 64.0\% & 7.2M  & 1.3G & 7.29 & 200K & 5.78$\times$ \\
    4 Regions & 64.0\% & 7.2M  & 1.3G & 7.55 & 200K & 5.78$\times$ \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-1.2em}
    \label{tab:ablation_num_models}
\end{table}


==> tables/flow_matching.tex <==
\begin{table}[h!]
    \centering
    \vspace{-1em}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
    \multicolumn{6}{c}{\textbf{CFM @ CIFAR10 32$\times$32}} \\
    \textbf{Method} & \textbf{\#Params $\downarrow$} & \textbf{MACs $\downarrow$} & \textbf{FID $\downarrow$} & \textbf{Iters} & \textbf{Speed-Up $\uparrow$} \\
    \midrule
    Unpruned & 35.7M & 6.1G & 6.70 & 100K & 1.00$\times$ \\
    \midrule
    Scratch & 9.0M  & 1.5G & 12.24 & 100K & 0.67$\times$ \\
    \textbf{EB} & 9.0M  & 1.5G & 11.53 & 100K & 2.03$\times$ \\
    \textbf{TA-EB} & 7.2M  & 1.3G & \TODO{XXX} & 50K & 2.69$\times$ \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-1.2em}
    \label{tab:ablation_num_models}
\end{table}


==> tables/position_table.tex <==

\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\begin{table}[ht]
    
    \centering
    \vspace{-0.9em} 
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc}
        \toprule
        \textbf{Method} & \textbf{Model Scheduling} & \textbf{Training Acceleration} & \textbf{Inference Acceleration} \\
        \midrule
        DDSM [ICLR'24] & \textcolor{darkgreen}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} \\ % Check marks
        OMS-DPM [ICML'23] & \textcolor{darkgreen}{\ding{51}} & \textcolor{red}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} \\ % Cross for Attribute 1
        DeepCache [CVPR'24] & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & \textcolor{darkgreen}{\ding{51}} \\ 
        \textbf{Our Method} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} & \textcolor{darkgreen}{\ding{51}} \\
        \bottomrule
    \end{tabular}
    } 
    \label{tab:position-table}
    \vspace{-1.2em}
\end{table}

==> tables/sm_ddpm_church_eb.tex <==
\begin{table}
\centering
\caption{EB Tickets with 50\% pruning rate on LSUN Church with 256 $\times$ 256 resolution using the DDPM \cite{ho2020denoising}. The best FID score is highlighted in \textbf{bold}. The ``Early Bird'' column denotes the pseudo-epoch of 1000 steps in which the subnetwork is sampled at.}
\vspace{-0.5em}
\scriptsize 
\setlength{\tabcolsep}{4pt} 
\renewcommand{\arraystretch}{1.2} 
\resizebox{\linewidth}{!}{ 
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multirow{2}[2]{*}{\tabincell{l}{\textbf{Pruning}\\\textbf{Metric}}} & \multicolumn{5}{c}{\textbf{DDPM @ LSUN Church (256$\times$256)}}
\\
\cmidrule(lr){2-6}
 & \textbf{\# Params} $\downarrow$ & \textbf{MACs} $\downarrow$ & \textbf{FID} $\downarrow$ & \textbf{Early Bird} & \textbf{Iters} \\
\midrule
\multirow{2}{*}{\shortstack[l]{Magnitude \\ Taylor}} 
& \multirow{2}{*}{19.7M} & \multirow{2}{*}{6.0G} & 37.6 & 14 & 800K\\
 & & & \tobeadded{???} & \tobeadded{???} & 800K\\
\bottomrule
\vspace{-2.5em}
\end{tabular}
}
\label{tab:ddpm_lsun_church}
\end{table}

==> tables/sm_imagenet_taeb.tex <==
\begin{table}[t]
    \centering
    \vspace{-1em}
    \caption{Results for \textbf{TA-EB} ImageNet-1K using the LDM \cite{rombach2021highresolution}. The number of iterations are recorded as the total number of iterations for the subnetwork with the longest training time.}
    \vspace{-0.5em}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Pruning Metric}} & \multicolumn{4}{c}{\textbf{LDM @ ImageNet (256$\times$256)}} \\
    \cmidrule(lr){2-5}
    & \textbf{\#Params $\downarrow$} & \textbf{MACs $\downarrow$} & \textbf{FID $\downarrow$} & \textbf{Iters} \\
    \midrule
    Magnitude & 267.5M & 117.3G & 44.63 & 50K \\
    Taylor & 267.5M & 117.3G & \tobeadded{???} & 50K \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:imagenet_ldm}
\end{table}

